ContourCNN: convolutional neural network for contour data classification

This paper proposes a novel Convolutional Neural Network model for contour data analysis (ContourCNN) and shape classification. A contour is a circular sequence of points representing a closed shape. For handling the cyclical property of the contour representation, we employ circular convolution layers. Contours are often represented sparsely. To address information sparsity, we introduce priority pooling layers that select features based on their magnitudes. Priority pooling layers pool features with low magnitudes while leaving the rest unchanged. We evaluated the proposed model using letters and digits shapes extracted from the EMNIST dataset and obtained a high classification accuracy.

==> abstract.tex <==

% \begin{abstract}

This paper proposes a novel Convolutional Neural Network model for contour data analysis (ContourCNN) and shape classification. A contour is a circular sequence of points representing a closed shape. For handling the cyclical property of the contour representation, we employ circular convolution layers. Contours are often represented sparsely. To address information sparsity, we introduce priority pooling layers that select features based on their magnitudes. Priority pooling layers pool features with low magnitudes while leaving the rest unchanged. We evaluated the proposed model using letters and digits shapes extracted from the EMNIST dataset and obtained a high classification accuracy.
% \end{abstract}

==> comments.tex <==
\begin{center}
\textbf{Author's response}
\end{center}

Dear reviewers,

We would like to thank you for reviewing our paper and taking the time to point out suggestions for improving it. 
We have recognized that the paper had some missing technical details, unclear figures, and that some decisions that need explanation.
Based on your comments and suggestion, we revised the paper, added the missing technical details, clarified figures, and exemplified some cases, and refined the explanation of several issues in the paper.

We have considered each comment individually as described below:

\subsection{Reviewer number 2}

We have addressed both of your comments. 
The ranges for Cartesian and the Polar representations were added to Section~\ref{sec:data_representation} and the typos in Section~\ref{sec:model} were fixed.

\subsection{Reviewer number 3}

\subsubsection{Problem with the literature methods and contribution of the paper} The main contribution of the paper over literature methods is that CNNs can learn the features. Traditional methods rely on hand-crafted features, which are rigid and pre-determined, i.e. once it is set, it can not adapt to the input data. Based on your comment we emphasised this point in the introduction.

\subsubsection{Using EMNIST rather than a more challenging dataset} Our intention is to introduce a new CNN model that deals with non-common space of contours, not to tackle a specific unsolved dataset. We chose the EMNIST dataset due to its size, simple objects (letters and digits). We needed a dataset to verify the applicability and initial performance of our model.
%and because it is easy to use- in so many words: you need to start somewhere.

\subsubsection{Separating the letters and digits subsets} This is done to avoid ambiguity among some of the letters and the digits. We revised Section~\ref{sec:dataset} to include this.

\subsubsection{Use of letter subset for comparison} Conducting the comparison between the activation layers, pooling layers, and the different data representations on both the digits and letters subsets would be redundant. We chose the letters subset over the digits' because it is more complex. The model was trained and tested on the official train and test split of the dataset. This was added to Section~\ref{sec:experiments}.

\subsubsection{... why not use the Alexnet itself}. Our intention is to introduce a new CNN model that deals with non-common space of contours which is not handled by AlexNet.

\subsubsection{There is no comparison with literature methods} Please refer to our response to comments 1 and 5.

\subsubsection{input of the model} This was clarified in Section~\ref{sec:model}.

\subsubsection{Extracting contour from images} The extraction algorithm we used was added to Section~\ref{sec:dataset}.

\subsubsection{The rest of the comments} All of the other issues you pointed out in the rest of your comments were fixed/addressed in the paper.


\subsection{Reviewer number 4}

\subsubsection*{General comments} 
\begin{itemize}
    \item Title was fixed
    \item We unified the mentions of the priority pooling layers
    \item We clarified the figures and labeled unlabeled axis-es. Regarding the confusion matrices; it was an issue of resolution. In order to solve this, we regenerated the confusion matrices in Figures~\ref{fig:contour_AL_confusion_matrix} and~\ref{fig:contour_letters_confusion_matrix}. Note that in order to regenerate the confusion matrices we retrained the models from scratch.
\end{itemize}


\subsubsection*{Specific Suggestions}
Here we would like to respond to a few comments. Regarding the rest, in most cases, we revised the paper as per your suggestions.

4. As per your suggestion we unified the notation of the depth. The reason D is mentioned in the description of equation (1), but not in it is that we needed a depth value to describe the kernel and the input sizes.

6. Yes, you understood correctly, kernel is applied on vertex with
the lowest magnitude and their adjacent neighbors. We used a kernel of size 3, however the kernel can be larger. We refined our explanation.


